Red Blue Set Cover Problem on Axis-Parallel Hyperplanes and Other Objects

Given a universe $\mathcal{U}=R \cup B$ of a finite set of red elements $R$, and a finite set of blue elements $B$ and a family $\mathcal{F}$ of subsets of $\mathcal{U}$, the \RBSC problem is to find a subset $\mathcal{F}'$ of $\mathcal{F}$ that covers all blue elements of $B$ and minimum number of red elements from $R$. We prove that the \RBSC problem is NP-hard even when $R$ and $B$ respectively are sets of red and blue points in ${\rm I\!R}^2$ and the sets in $\mathcal{F}$ are defined by axis-parallel lines i.e, every set is a maximal set of points with the same $x$ or $y$ coordinate. We then study the parameterized complexity of a generalization of this problem, where $\mathcal{U}$ is a set of points in ${\rm I\!R}^d$ and $\mathcal{F}$ is a collection of set of axis-parallel hyperplanes in ${\rm I\!R}^d$, under different parameterizations. For every parameter, we show that the problem is fixed-parameter tractable and also show the existence of a polynomial kernel. We further consider the \RBSC problem for some special types of rectangles in ${\rm I\!R}^2$.

==> PAsection.tex <==


\begin{table}[h!]
	\centering
	\begin{tabular}{|c|c|c|c|}
		\hline
		\textbf{Parameter} & \textbf{Gen- RBSC}  & \textbf{AX-RBSC} & \textbf{GenAX-RBSC}  \\ 
		\hline
		$k_r$ & Para-NP hard & FPT & Para-NP hard \\  
		\hline
		$b$& W-hard & FPT & FPT\\  
		\hline
		$l$& FPT & FPT & FPT\\  
		\hline
		$k_l$& W-hard & FPT & FPT\\  
		\hline
		$r$& Para-NP hard & FPT& Para-NP hard \\  
		\hline 
		
	\end{tabular}
	\vspace{0.2cm}
	\caption{Comparision study of Gen-RBSC, GenAxis-parallel and Axis-parallel RBSC }
	\label{TT1}
\end{table}

==> Para_red.tex <==


We design a parameterized algorithm and a kernel for Gen-RBSC axis parallel lines when parameterized by the size $r$. We enumerate all possible subsets of input red points and for each subset, we check in polynomial time whether it covers all blue points and at most $k$ red points. The algorithm runs in time $O(2^{r} (|U | + |F |)$. The same algorithm works in higher dimensions also. Thus the running time is the same  in $R^d$ also.

	
%\textbf{Parameterizing by $k_r$: kernalization}\\
\begin{lemma}
	if $(L',k)$ is yes  instance and none of the reduction rules are applicable to the  Instance $(L',k)$, then $|B|=(2r)^2$, $|L|=2r$, and $|k|={l}^2$ in $R^2$
\end{lemma}

\begin{proof}		
	We cannot apply reduction rules anymore on $(L',k)$, every line contains at least one red point. One red point is covered by at most two lines (either horizontal or vertical). Hence the number of lines are passing through one red point is two. Then the number of lines $l$ is $2r$. Similarly, one line contains at most $b$ blue points. There are at most $l$ lines. Hence the number of blue points is $O(l^2)$. i.e,  $O((2r)^2)$
\end{proof}

Similar to $R^2$, if $(L',k)$ is yes  instance and none of the reduction rules are applicable to the  Instance $(L',k)$, then $|B|=l^d$, and $|l|=dr$ in $R^d$

